Towards Accurate Labeling of Android Apps for Reliable Malware Detection

In training their newly-developed malware detection methods, researchers rely on threshold-based labeling strategies that interpret the scan reports provided by online platforms, such as VirusTotal. The dynamicity of this platform renders those labeling strategies unsustainable over prolonged periods, which leads to inaccurate labels. Using inaccurately labeled apps to train and evaluate malware detection methods significantly undermines the reliability of their results, leading to either dismissing otherwise promising detection approaches or adopting intrinsically inadequate ones. The infeasibility of generating accurate labels via manual analysis and the lack of reliable alternatives force researchers to utilize VirusTotal to label apps. In the paper, we tackle this issue in two manners. Firstly, we reveal the aspects of VirusTotal's dynamicity and how they impact threshold-based labeling strategies and provide actionable insights on how to use these labeling strategies given VirusTotal's dynamicity reliably. Secondly, we motivate the implementation of alternative platforms by (a) identifying VirusTotal limitations that such platforms should avoid, and (b) proposing an architecture of how such platforms can be constructed to mitigate VirusTotal's limitations.

==> backup/5evaluation.tex <==
\section{Evaluating Maat}
\label{sec:evaluation}

As discussed in \autoref{sec:introduction}, the accurate labeling of previously-analyzed and detected apps is fundamental for the effectiveness of detection methods. 
So, the quality of labeling strategies can be assessed in terms of (a) their abilities to assign labels to previously-analyzed apps (e.g., based on their \VT{} scan reports) that accurately reflect their ground truth, and (b) the extent to which such accurate labeling contributes to the effectiveness of detection methods against out-of-sample apps. 
In this section, we evaluate the performance of threshold-based labeling strategies versus \Maat{}'s \gls{ml}-based labeling strategies according to the aforementioned two criteria. 
In \autoref{subsec:evaluation_accuracy}, we verify whether \Maat{}'s \gls{ml}-based labeling strategies trained at one point in time can maintain labeling accuracies in the future that rival those achieved using threshold-based labeling strategies that adopt the current optimal thresholds. 
The second set of experiments in \autoref{subsec:evaluation_enhancing} compares the impact of threshold-based labeling strategies versus that of \Maat{}'s \gls{ml}-based labeling strategies on the effectiveness of \gls{ml}-based detection methods against out-of-sample apps over time. 

\subsection{Accurately Labeling Apps}
\label{subsec:evaluation_accuracy}
The main objective in this set of experiments is to verify whether \gls{ml}-based labeling strategies trained at one point in time can sustain a similar labeling accuracy using \VT{} scan reports downloaded in the future. 
If true, then unlike their threshold-based counterparts, \Maat{} \gls{ml}-based labeling strategies do not need to be re-trained regularly to accommodate for \VT{}'s dynamicity. 
So, we trained \Maat{} \gls{ml}-based labeling strategies using \VT{} scan reports of apps in the \emph{AMD+GPlay} dataset downloaded on \earliestDate{}, and used the trained strategies to label apps in the test datasets \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets between July 5$^{th}$, 2019 and \futureDate{}. 
In the experiments, we used \gls{ml}-based labeling strategies that use the two types of features mentioned in \autoref{subsec:maat_features} (i.e., engineered versus naive) and trained using the technique of grid search. 
We also included labeling strategies that used the \texttt{SelectFromModel} technique to select the most informative features. 
For readability, we shorten the names of \gls{ml} labeling strategies in the following manner: engineered and naive features are referred to as \texttt{Eng} and \texttt{Naive}, respectively, grid search is referred to as \texttt{GS}, and strategies that use selected features are referred to using \texttt{Sel}. 
For example, a labeling strategy that uses selected engineered features and the grid search techniques will be referred to as \texttt{Eng Sel GS}. 

\autoref{fig:mccs_over_time_2} depicts an example of the results we are discussing in this section. 
In this figure, we compare the labeling performance of the \gls{ml}-based labeling strategies trained using scan reports from \earliestDate{} against two types of threshold-based labeling strategies. 
The solid red line depicts the performance of threshold-based strategies using the optimal threshold at each scan date identified as follows. 
At each scan date, we calculated the labeling accuracy of each threshold between one and 60 against apps in the \emph{AMD+GPlay} dataset. 
The threshold that yields the best \gls{mcc} scores is considered as the optimal threshold for this scan date. 
For example, using scan reports of the \emph{AMD+GPlay} dataset re-scanned and downloaded on July 5$^{th}$, 2019, the optimal threshold was found to be 12 \VT{} scanners. 
So, the labeling strategy used to label apps in the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets on July 5$^{th}$, 2019 is \texttt{vt$\geq$12}.  
The other type of threshold-based labeling strategies we use (dashed orange line) depicts strategies that use the optimal threshold that would achieve the best \gls{mcc} scores on each of the test datasets. 
These thresholds are found by trying different thresholds on the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets. 
They are meant to simulate a scenario in which a researcher always manages to find the thresholds that yield the best possible \gls{mcc} scores on the test datasets. 
Effectively, the performance of these thresholds depicts an upper bound on the performance of threshold-based labeling strategies on the test datasets. 

The performance of the brute-forced thresholds in \autoref{fig:mccs_over_time_2} and \autoref{fig:mccs_over_time_2_selected} demonstrates the main limitation of the brute forcing approach to finding the optimal threshold of \VT{} scanners at a given point in time: in order for the thresholds obtained by brute-forcing all possible values to generalize to new Android malware, the dataset used to find these optimal thresholds needs to be temporally diverse. 
Given that the \emph{AMD+GPlay} dataset does not contain apps developed in 2019, the identified thresholds were high (i.e., between 10 and 13 scanners), and could not accurately label apps in the \emph{Hand-Labeled 2019} dataset. 
As for \Maat{}'s \gls{ml}-based labeling strategies, with a few exceptions, we found that (a) their \gls{mcc} scores mimicked that of the best possible threshold at each scan date and (b) had stable \gls{mcc} scores over the period of time between July 5$^{th}$, 2019 and \futureDate{}. 
Recall that for all scan dates, we used \gls{ml}-based labeling strategies trained using \VT{} scan reports that date back to different months in \earliestDate{} and using a dataset of older apps (i.e., \emph{AMD+GPlay}). 
This means that using \VT{} scan reports of older apps, such labeling strategies can maintain decent, stable labeling accuracies for at least a year even against newer apps.  

\begin{figure*}
\centering
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Eng_GS_Hand-Labeled.pgf}}
 	 \caption{\texttt{Eng GS} on \emph{Hand-Labeled}}
   	\label{fig:mccs_over_time_2_eng_gs_handlabeled}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Naive_GS_Hand-Labeled.pgf}}
 	 \caption{\texttt{Naive GS} on \emph{Hand-Labeled}}
   	\label{fig:mccs_over_time_2_naive_gs_handlabeled}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Eng_GS_Hand-Labeled2019.pgf}}
 	 \caption{\texttt{Eng GS} on \emph{Hand-Labeled 2019}}
   	\label{fig:mccs_over_time_2_eng_gs_handlabeled2019}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Naive_GS_Hand-Labeled2019.pgf}}
 	 \caption{\texttt{Naive GS} on \emph{Hand-Labeled 2019}}
   	\label{fig:mccs_over_time_2_naive_gs_handlabeled2019}
\end{subfigure}
\caption{The labeling accuracies achieved by \Maat{}'s \gls{ml}-based labeling strategies \texttt{Eng GS} and \texttt{Naive GS} trained with scan reports downloaded in between \earliestDate{} and June 21$^{st}$, 2019 against apps in the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets over time.}
\label{fig:mccs_over_time_2}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Eng_Sel_GS_Hand-Labeled.pgf}}
 	 \caption{\texttt{Eng Sel GS} on \emph{Hand-Labeled}}
   	\label{fig:mccs_over_time_2_eng_sel_gs_handlabeled}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Naive_Sel_GS_Hand-Labeled.pgf}}
 	 \caption{\texttt{Naive Sel GS} on \emph{Hand-Labeled}}
   	\label{fig:mccs_over_time_2_naive_sel_gs_handlabeled}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Eng_Sel_GS_Hand-Labeled2019.pgf}}
 	 \caption{\texttt{Eng Sel GS} on \emph{Hand-Labeled 2019}}
   	\label{fig:mccs_over_time_2_eng_sel_gs_handlabeled2019}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
	\centering
	\scalebox{0.42}{\input{figures/Line_Thresholds_ML_Naive_Sel_GS_Hand-Labeled2019.pgf}}
 	 \caption{\texttt{Naive Sel GS} on \emph{Hand-Labeled 2019}}
   	\label{fig:mccs_over_time_2_naive_sel_gs_handlabeled2019}
\end{subfigure}
\caption{The labeling accuracies achieved by \Maat{}'s \gls{ml}-based labeling strategies \texttt{Eng Sel GS} and \texttt{Naive Sel GS} trained with scan reports downloaded in between \earliestDate{} and June 21$^{st}$, 2019 against apps in the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets over time.}
\label{fig:mccs_over_time_2_selected}
\end{figure*}

We made the following observations based on the \gls{mcc} scores in \autoref{fig:mccs_over_time_2} and \autoref{fig:mccs_over_time_2_selected}. 
Firstly, with the exception of \gls{ml}-based labeling strategies trained using scan reports dating back to \earliestDate{}, the performance of labeling strategies using engineered features (i.e., \texttt{Eng GS} and \texttt{Eng Sel GS}), significantly deteriorates on the \emph{Hand-Labeled 2019} dataset. 
However, labeling strategies trained with \texttt{Eng Sel GS} seem to have higher scores than their counterparts trained with \texttt{Eng GS}, which is more evident against the \emph{Hand-Labeled 2019} dataset, as seen in \autoref{fig:mccs_over_time_2_eng_gs_handlabeled2019} versus \autoref{fig:mccs_over_time_2_eng_sel_gs_handlabeled2019}. 
Secondly, in contrast, the \gls{mcc} scores of labeling strategies using the naive features appears to be more stable than their counterparts using engineered features on both test datasets \emph{Hand-Labeled} and \emph{Hand-Labeled 2019}. 
Similar to the case with engineered features, the selected naive features \texttt{Naive Sel GS} enable the \gls{ml}-based labeling strategies to achieve higher \gls{mcc} scores and maintain almost the same performance over time regardless of when the labeling strategy was trained. 
Lastly, the performance of both types of features seems to fluctuate over time, albeit not with the same rate or severity. 
Using selected features seems to decrease or remove such fluctuations, especially upon using the naive feature set. 
To understand the reasons that led to the manifestations of such behaviors, we studied the structures of the random forests, which constitute \Maat{}'s \gls{ml}-based labeling strategies, including the features they learn, their depth, and how they classify apps based on their \VT{} scan reports. 

\subsubsection{Features Learned by ML-based Labeling Strategies}

\paragraph{\textbf{Engineered Features}.}

In \autoref{fig:eng_gs_trees_2018}, we show an example of the decision trees trained using engineered features based on \VT{} scan reports of the training dataset \emph{AMD+GPlay} downloaded in \earliestDate{}. 
We found that on this date, the decision trees within the train random forests had almost identical structures and features, whether trained using the full or selected corpus of the engineered feature set (i.e., \texttt{Eng GS} or \texttt{Eng Sel GS}). 
As seen in the figure, the tree uses a mixture of the feature categories mentioned in \autoref{subsec:maat_features}, namely attributes found in the apps' scan reports (e.g., \emph{positives} and \emph{total}), features that indicate the age of an app, and the verdicts of some \VT{} scan reports (e.g., \texttt{Babable} and \texttt{MAX}). 
The tree's structure allows it to accurately classify Android apps in the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets as follows. 
First, the left subtree classifies apps after checking the ratio of \emph{positives} to \emph{total} attributes in the scan report, which allows it to cater to newly-developed malicious apps. 
That is if the number of scanners is less than 2 (i.e., \emph{positives}$\leq$2.5) and the total number of scanners in the scan reports is less than 24 (i.e., \emph{total}$\geq$24.5), the tree assumes that the app is newly-developed yet around 9\% of scanners deem it malicious, and in turn labels the app as malicious. 
Otherwise, if the total number of scanners is more 24, the tree considers the app's scan report to be mature (i.e., old app), yet only a small subset of scanners deem it as malicious; in this case, the tree considers the \emph{positives} to be false positives and deems the app as benign. 
For our test datasets, we found that this subtree is effective at classifying benign apps and minimizing false positives.  

\begin{figure}
	\centering
	\caption{An example of a decision tree trained using grid search and all engineered features \texttt{Eng GS} extracted from apps in the \emph{AMD+GPlay} dataset in \earliestDate{}.}
	\label{fig:eng_gs_trees_2018}
	\includegraphics[scale=0.33]{figures/trees_eng_gs/tree_18_eng_gs_trees_2018}
\end{figure}

The tree's right subtree checks the \emph{positives} attribute again and labels apps as malicious if more than 16 scanners deem an app malicious. 
This check helps identify old malicious apps whose \VT{} scan reports have matured to include values of \emph{positives} higher than these thresholds. 
As per \futureDate{}, 99.65\% of the malicious apps in the \emph{AMD+GPlay} dataset and 67\% of those in the \emph{Hand-Labeled} test dataset had \emph{positives} values greater than or equal to 16. 
However, this check does not help classify newly-developed malicious apps, such as those in the \emph{Hand-Labeled 2019} dataset. 
In this case, the tree checks the verdict of the \texttt{Babable} scanner. 
If the scanner deems an app malicious, it checks the verdict of another scanner (i.e., TrendMicro's \texttt{MAX}), and deems the app as malicious or benign according to this scanner's verdict. 
Effectively, the tree deems the app as malicious if two scanners, which we found to be among the correct scanners for the \emph{AMD+GPlay} and \emph{Hand-Labeled 2019} datasets in \autoref{subsec:maat_correctness}, deem the app malicious. 
If \texttt{Babable} finds the app benign, the tree makes a final check about the age of the app being less than 7.3 years. 
However, this check can be ignored because, regardless of the outcome, the tree assigns the app to the majority class in this subtree, which is malicious. 

For apps in our test datasets, we found that benign and malicious apps are labeled according to the following decision paths. 
On the one hand, benign apps are classified using the left subtree after satisfying the conditions that \emph{positives}$\leq 2\ AND$ \emph{total} $\geq 25$. 
On the other hand, malicious apps in the \emph{Hand-Labeled} dataset were labeled malicious after satisfying the conditions \emph{positives}$\geq 3\ AND$ \emph{positives}$\geq 16\ AND$. 
However, given their novelty, malicious apps in the \emph{Hand-Labeled 2019} datasets were labeled malicious after satisfying the conditions \emph{positives}$\geq 3\ AND$ \texttt{Babable} $\leq 0.0$. 
Upon further investigation of the app's scan reports, we found that they are correctly classified whenever \VT{} excludes \texttt{Babable} from their scan reports. 
Furthermore, we found that the \texttt{MAX} scanner never detected any of those apps. 
So, effectively, the apps were labeled as malicious if the check \texttt{Babable} $==-1$ is true. 
Although this check is effective at labeling apps as malicious, it does not make sense to label apps based on the absence of a scanner. 
This is an example of how \VT{}'s first limitation of including and excluding scanners in the scan reports of apps might impact the way \Maat{}'s \gls{ml}-based trees are trained. 

As for the performance of \gls{ml}-based labeling strategies trained at different points in time, we found that the main reason behind their underperformance is their shallowness. 
We found that--whether they use all of the engineered features or a selected subset of them--all decision trees in random forests trained between April 12$^{th}$, 2019 and June 7$^{th}$, 2019 employ only one check making them shallow trees of depth one. 
With this depth, the tree is unable to represent apps in the training dataset, which is apparent in the impurity of the leaf nodes. 
For example, the left leaf node of \autoref{fig:eng_gs_trees_april12_1}'s second tree shows that 55\% of the remaining apps are benign, and 45\% are malicious; apps will be labeled as benign because the majority class, in this case, is benign. 
Later in this section, we explain why trees of depth one can be trained using either type of features, viz.\ engineered and naive. 

\begin{figure*}
\centering
\begin{subfigure}{0.46\textwidth}
	\centering
    \includegraphics[scale=0.25]{figures/trees_eng_gs/tree_6_eng_gs_trees_2019-04-12}
    \includegraphics[scale=0.25]{figures/trees_eng_gs/tree_66_eng_gs_trees_2019-04-12}
     \caption{Using \textbf{all} engineered features}
     \label{fig:eng_gs_trees_april12_1}
\end{subfigure}
\begin{subfigure}{0.46\textwidth}
	\centering
    \includegraphics[scale=0.25]{figures/trees_eng_gs/tree_14_eng_sel_gs_trees-2019-04-12}
    \includegraphics[scale=0.25]{figures/trees_eng_gs/tree_22_eng_sel_gs_trees-2019-04-12}
     \caption{Using \textbf{selected} engineered features}
     \label{fig:eng_sel_gs_trees_apr12}
\end{subfigure}
\caption{Four randomly selected decision trees in the \gls{ml}-based labeling strategies' random forests trained using grid search and engineered features \texttt{Eng GS} extracted from \VT{} scan reports of apps in the \emph{AMD+GPlay} dataset downloaded on April 12$^{th}$, 2019.}
\label{fig:eng_gs_trees_april12}
\end{figure*}

Despite being all of the depth one, some of the decision trees in these random forests are more effective than others. 
For example, the decision tree in \autoref{fig:eng_gs_trees_april12} uses the verdict of \texttt{ESET-NOD32} to classify apps, which we showed in \autoref{subsec:maat_correctness} to be a consistently correct scanner. 

Unfortunately, other decision trees trained on April 12$^{th}$, 2019 using all engineered features are subjective and fail on their own to represent patterns found in either the training dataset \emph{AMD+GPlay} or the test datasets. 
For example, the second decision tree (from the left) relies on the \emph{checks-gps} tag to label apps. 
This \VT{} tag does not help discern the malignancy of an app, especially since using the \gls{gps} module is common among malicious and benign apps alike. 

Using a selected subset of the engineered features yields decision trees that are confident about their labels, as indicated by the Gini values in the leaf nodes. 
Checks that did not yield confident labels, such as the \VT{} tags and the permissions requested by an app, are excluded. 
The decision trees rely on either the verdicts of scanners that we found to be correct in \autoref{subsec:maat_correctness} on the \emph{AMD+GPlay} dataset or scan report attributes such as \emph{positives} and \emph{total}. 
While selecting features helped increase the performance of \gls{ml}-based labeling strategies using engineered features, they still failed to perform well on the \emph{Hand-Labeled 2019} dataset. 
The reason for this is two-fold. 
Firstly, relying on the verdicts of only one scanner makes the decision tree susceptible to \VT{}'s dynamicity and the resulting first limitation. 
Regardless of the correctness and stability of the scanner, it risks being excluded from the scan reports of apps, which forces a decision tree to label all apps as benign. 
This explains the fluctuation of \texttt{Naive GS} and \texttt{Naive Sel GS} on this dataset over time. 
Secondly, the scan report attributes of \emph{positives} and \emph{total} are also susceptible to \VT{}'s dynamicity. 
More importantly, using threshold values such as five might suit the older apps in the \emph{AMD+GPlay} dataset, where the malicious apps have \emph{positives} values usually greater than ten and benign values of zero \emph{positives}. 
However, such low values may not generalize to newer apps where only a small subset of \VT{} scanners might already recognize their malignancies.

\paragraph{\textbf{Naive Features}.}

Using naive features and grid search \texttt{Naive GS}, we found that the random forests that make up the \gls{ml}-based labeling strategies had three different structures and depths. 
The random forest trained using this type of features on \earliestDate{} had depths of ten. 
For readability, in \autoref{fig:eng_gs_trees_2018}, we show parts of an example decision tree that belongs to this random forest. 
The decision tree in the figure checks the verdicts of different \VT{} scanners, some of which we found to be correct, such as \texttt{Fortinet} and \texttt{Ikarus}, and others that we found to be hesitant, such as \texttt{Cyren}. 
However, checking the verdicts of these different scanners yield pure leaf nodes that are confident about the class of an app (i.e., Gini index of zero). 
Although this random forest had decent and stable \gls{mcc} scores on both test datasets, one can notice the presence of checks similar to the \texttt{Babable} example with engineered features, namely checks that rely on the absence of a scanner's verdict. 
For example, the fourth node and its two child nodes check whether the verdicts of the scanners \texttt{Jiangmin}, \texttt{VIPRE}, and \texttt{Kingsoft} do not exist in the scan report being processed. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[scale=0.25]{figures/trees_naive_gs/tree_81_naive_gs_trees_2018}
		\caption{Using \textbf{all} naive features}
		\label{fig:naive_gs_trees_2018_all}
	\end{subfigure}
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[scale=0.25]{figures/trees_naive_gs/tree_11_naive_sel_gs_trees-2018}
		\caption{Using \textbf{selected} naive features}
		\label{fig:naive_gs_trees_2018_selected}
	\end{subfigure}
	\caption{Two decision trees trained using grid search and naive features \texttt{Naive GS} and \texttt{Naive Sel GS} extracted from apps in the \emph{AMD+GPlay} dataset in \earliestDate{}.}
	\label{fig:naive_gs_trees_2018}
\end{figure}

This type of checks does not exist in decision trees trained using selected naive features. 
As seen in \autoref{fig:naive_gs_trees_2018_selected}, decision trees in the \texttt{Naive Sel GS} random forests had depths of four and their structures were different from the ones trained with all naive features in two aspects. 
First, they relied on the verdicts of correct scanners. 
That is we did not find any decision trees that rely on the verdicts of \VT{} scanners, such as \texttt{GData}, \texttt{Alibaba}, or \texttt{Kingsoft}. 
Second, they relied on the verdicts of scanners that are included in the scan reports and checked whether each scanner deemed an app as malicious or benign rather than whether the scanner's verdicts were absent from the scan report. 
The performance of \texttt{Naive Sel GS} \gls{ml}-based labeling strategies mimicked that of their \texttt{Naive GS} counterparts on the \emph{Hand-Labeled} dataset. 
However, on the newer \emph{Hand-Labeled 2019} dataset, that performance decreases in terms of \gls{mcc} scores by about 0.1, albeit remaining stable.

The depth of four does not seem to hinder the performance of \gls{ml}-based labeling strategies using naive features. 
As seen in \autoref{fig:naive_gs_trees}, using an average depth of four, the labeling strategies that used both all and selected naive features had \gls{mcc} scores  that (a) were stable over time, and (b) matched and in some cases outperformed those of threshold-based labeling strategies using the current optimal threshold.
The primary difference between random forests trained using \texttt{Naive GS} and \texttt{Naive Sel GS} was the utilization of correct and stable \VT{} scanners. 
On the one hand, \texttt{Naive GS} decision trees relied on the verdicts of a mixture of correct scanners (e.g., \texttt{Sophos}, \texttt{ESET-NOD32}, and \texttt{NANO-Antivirus}) and other less reliable scanners to label apps.
On the other hand, \texttt{Naive Sel GS} exclusively relied on the verdicts of correct and stable scanners, as identified in \autoref{sec:maat}. 
In both cases, we noticed that the deeper the decision trees grow, the lower the number of malicious apps that need to be labeled. 
For example, in both decision trees in \autoref{fig:naive_gs_trees}, by the time the last check is performed, less than 1\% of the malicious apps remain to be classified. 
So, it seems that the checks employed by the decision trees attempt to identify malicious apps first, and the remaining apps are being classified as benign. 

\begin{figure*}
\centering
\begin{subfigure}[b]{0.46\textwidth}
	\centering
    \includegraphics[scale=0.30]{figures/trees_naive_gs/tree_6_naive_gs_trees_2019-04-12}
     \caption{Using \textbf{all} naive features}
     \label{fig:naive_gs_trees_april}
\end{subfigure}
\begin{subfigure}[b]{0.46\textwidth}
	\centering
    \includegraphics[scale=0.30]{figures/trees_naive_gs/tree_30_naive_sel_gs_trees-2019-04-12}
     \caption{Using \textbf{selected} naive features}
     \label{fig:naive_sel_gs_trees_april}
\end{subfigure}
\caption{Two randomly selected decision trees in the \gls{ml}-based labeling strategies' random forests trained using grid search and naive features \texttt{Naive Sel GS} extracted from \VT{} scan reports of apps in the \emph{AMD+GPlay} dataset downloaded on April 12$^{th}$, 2019}
\label{fig:naive_gs_trees}
\end{figure*}

As for the performance of both types of \gls{ml}-based labeling strategies on the test datasets, we noticed that labeling strategies using \texttt{Naive Sel GS} had fewer fluctuations in \gls{mcc} scores over time on both datasets that its \texttt{Naive GS} counterpart.  
Moreover, the mediocre performance of \gls{ml}-based labeling strategies trained using \texttt{Naive GS} on April 26$^{th}$, 2019 increases upon using selected naive features. 
The reason for that we found is that using selected naive features (i.e., \texttt{Naive Sel GS}), the depth of the random forests increases from one to four to resemble the structure of other \texttt{Naive Sel GS} random forests. 
We visualize the structure of \texttt{Naive GS} and \texttt{Naive Sel GS} \gls{ml}-based labeling strategies trained on this date in \autoref{fig:naive_gs_trees_apr26}.
On the one hand, random forests trained using all naive features (seen in \autoref{fig:naive_all_gs_trees_apr26}) result into decision trees that employ only one check of different \VT{} scanners. 
The more reliable and correct the scanner is (e.g., \texttt{NANO-Antivirus} or \texttt{SymantecMobileInsight)}, the more confident are the labeling decisions. 
Decision trees that rely on the verdicts of scanners, such as \texttt{Baidu}, are likely to yield unconfident labels. 
On the other hand, using selected naive features yields random forests with decision trees of an average length of four, which rely on the verdicts of four scanners, most of which we found to be correct and stable. 

\begin{figure*}
\centering
\begin{subfigure}[b]{0.45\textwidth}
	\centering
    \includegraphics[scale=0.3]{figures/trees_naive_gs/tree_88_naive_gs_trees_2019-04-26}
    \includegraphics[scale=0.3]{figures/trees_naive_gs/tree_89_naive_gs_trees_2019-04-26}
     \caption{Using \textbf{all} naive features}%April 12$^{th}$, 2019}
     \label{fig:naive_all_gs_trees_apr26}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
	\centering
    \includegraphics[scale=0.3]{figures/trees_naive_gs/tree_8_naive_sel_gs_trees-2019-04-26}
    %\includegraphics[scale=0.25]{figures/trees_naive_gs/tree_66_naive_sel_gs_trees-2019-04-26}
     \caption{Using \textbf{selected} naive features}%June 7$^{th}$, 2019}
     \label{fig:naive_sel_gs_trees_apr26}
\end{subfigure}
\caption[Three randomly selected decision trees in the \gls{ml}-based labeling strategies' random forests trained using grid search and naive features extracted from \VT{} scan reports of apps in the \emph{AMD+GPlay} dataset downloaded on April 26$^{th}$, 2019.]{Three randomly selected decision trees in the \gls{ml}-based labeling strategies' random forests trained using grid search and naive features extracted from \VT{} scan reports of apps in the \emph{AMD+GPlay} dataset downloaded on April 26$^{th}$, 2019. The two trees on the left were trained using \textbf{all} naive features \texttt{Naive GS} and the tree on the right was trained using \textbf{selected} naive features \texttt{Naive Sel GS}.}
\label{fig:naive_gs_trees_apr26}
\end{figure*}

So, we can sum up the results of this section as follows. 
First, we found that naive features train \gls{ml}-based labeling strategies have higher and more stable \gls{mcc} scores on both test datasets than their counterparts trained using engineered features. 
Second, for both types of features, we found that selecting the most informative features boosts the labeling accuracies of \gls{ml}-based labeling strategies and relatively smoothens the fluctuations of their \gls{mcc} scores over time. 
Third, in associating the labeling accuracies with the structure of decision trees in the random forests constituting \gls{ml}-based labeling strategies, we found that decision trees that rely on the verdicts of between three and four \VT{} scanners, which we found to be correct and stable on the training dataset \emph{AMD+GPlay}, yields the best and most stable \gls{mcc} scores. 
In the next section, we attempt to explain what controls the structure of the trained random forests and the role that \VT{}'s dynamicity plays in this. 

\subsubsection{Sensitivity to \VT{}'s Dynamicity}

In \autoref{subsec:maat_overview}, we mentioned that we use the technique of grid search to find the hyperparameters that yield the most accurate random forests that constitute \Maat{}'s \gls{ml}-based labeling strategies. 
One of those hyperparameters controls the maximum depth each decision tree in the random forest is allowed to grow (i.e., \emph{max\_depth}). 
We varied the value of \emph{max\_depth} to be one, four, ten, and \texttt{None}, and allowed the technique of grid to identify the value that yields the best validation accuracy ($\frac{TP+TN}{P+N}$) achieved using the technique of cross-validation, which we set to be ten-fold. 
In our case, this accuracy is calculated by splitting the scan reports of apps in the \emph{AMD+GPlay} dataset into ten folds, train the random forests using nine of those, and using the remaining one-tenth as validation dataset. 
The final validation accuracy is an average of all ten accuracies achieved on the ten validation datasets. 

We found that the validation accuracies achieved by random forests of different depths are very close to one another. 
For example, for \texttt{Naive GS} \gls{ml}-based labeling strategies trained on April 26$^{th}$, 2019, we found that the validation accuracies achieved by random forests with \emph{max\_depth} values of one, four, ten, and \texttt{None} were 1.0, 0.9999794703346335, 0.9999794703346335, and 0.9999589490951507, respectively. 
Based on those values and despite the insignificant difference in validation accuracies, the grid search algorithm suggested the random forests with \emph{max\_depth} of one as the best random forest. 
So, what causes this small difference? 
The difference between both values is 0.00002053. 
This means that out of one tenth of the total number of apps in the \emph{AMD+GPlay} datasets (i.e., $48,715\times0.1=4,871$), an average of 0.10 (i.e., $4,871\times 0.00002053=0.100011895$) apps gets misclassified in the validation dataset. 
Since this value is an average, we can assume that at some validation folds, a few apps out of 4,871 are misclassified. 

In this case of \texttt{Naive GS} \gls{ml}-based labeling strategies, since they rely on the verdicts given by \VT{} scanners, the frequent change in the verdicts of scanners (i.e., \VT{}'s first limitation), is expected to have an impact on the feature vectors used to train the labeling strategies' random forests. 
In fact, we found that between April 12$^{th}$, 2019, and April 26$^{th}$, 2019 only 15\% of the apps in the \emph{AMD+GPlay} dataset had the exact same verdicts. 
Furthermore, between these two dates, almost 85\% of the apps had at least one verdict change, 51.65\% hat at least two verdicts change, and 23.4\% had at least three verdicts change. 
Examining these differences between all other training dates (i.e., between \earliestDate{} and June 21$^{st}$, 2019), yielded very similar percentages. 
Nonetheless, these percentages do not reveal which verdicts have been changed. 
So, the likely scenario on April 26$^{th}$, 2019 is that the verdicts in the \VT{} scan reports of apps in the \emph{AMD+GPlay} dataset changed in a manner that gave a slight edge to random forests with \emph{max\_depth} of one enough to make them be chosen as the best random forests. 
In that sense, the dynamicity of \VT{} can impact the performance of \Maat{}'s \gls{ml}-based labeling strategies' random forests yielding ones with shallow decision trees that perform well on the training dataset, yet fail to generalize to test datasets. 

Another aspect of the \gls{ml}-based labeling strategies' sensitivity to \VT{}'s dynamicity is related to the platform's third limitation, namely that it sometimes utilizes inadequate scanners and versions of scanners that are not designed to cater to Android malware. 
In particular, this limitation affected \texttt{Naive Sel GS}, which relies on the verdicts of scanners to label apps. 
As seen in \autoref{subsec:maat_correctness}, some scanners, such as \texttt{BitDefender}, had better labeling accuracy in \earliestDate{} before their versions were altered by \VT{}. 
Consequently, \texttt{Naive Sel GS} labeling strategies trained using \earliestDate{} versions of apps in the \emph{AMD+GPlay} dataset might include scanners that were correct and stable back then (e.g., \texttt{Trustlook} and \texttt{Avira}). 
These scanners ceased to be correct and stable and, hence, were not able to help label apps accurately in the test datasets according to their scan reports downloaded at different points in time in 2019. 

\subsection{Enhancing Detection Methods}
\label{subsec:evaluation_enhancing}

The second criterion we use to evaluate the applicability of \Maat{}'s \gls{ml}-based labeling strategies is their ability to contribute to training more effective \gls{ml}-based detection methods. 
In \autoref{sec:introduction}, we discussed that inaccurate labeling might have a negative impact on the detection performance on potentially effective detection methods. 
By addressing this issue of labeling accuracy, we can contribute to helping the research community focus on developing effective detection methods rather than being consumed by devising labeling strategies that accurately label apps in their training datasets. 
Our main hypothesis in this section is that accurate labeling should, in turn, lead to more effective detection of out-of-sample apps. 
So, since \Maat{}'s \gls{ml}-based labeling strategies managed to accurately label apps in the test datasets over a period of time, we hypothesize that they can accurately label apps in the \emph{AndroZoo} dataset and lead to training \gls{ml}-based detection methods that accurately label apps in those test datasets, viz.\ \emph{Hand-Labeled}, and \emph{Hand-Labeled 2019} datasets. 

We focus on \gls{ml}-based detection methods given their popularity within the academic community \cite{pendlebury2018enabling,suarez2017droidsieve,tam2017evolution,yang2017malware,arshad2016android}. 
In essence, we train different \gls{ml} classifiers using static features extracted from the \emph{AndroZoo} dataset, which depict information about the apps' components \cite{sato2013detecting,sanz2013puma}, the permissions they request \cite{arp2014drebin,wu2012droidmat}, the \gls{api} calls found in their codebases \cite{sachdeva2018android,zhou2013fast}, and the compilers used to compile them \cite{stazzere2016detecting}. 
The feature vectors are then labeled using different threshold-based and \gls{ml}-based labeling strategies. 
We test the detection abilities of such classifiers by assessing their ability to label apps in the \emph{Hand-Labeled}, and \emph{Hand-Labeled 2019} datasets correctly. 
For readability, we use the shorter term \emph{classifier was labeled} instead of \emph{classifier whose feature vectors were labeled}. 

There is a plethora of approaches to using static features and \gls{ml} algorithms to detect Android malware. 
We utilize a detection method that is renowned in the research community and has been used by different researchers as a benchmark ~\cite{pendlebury2019}, namely \emph{Drebin} ~\cite{arp2014drebin}. 
The \emph{Drebin} approach comprises three components: a linear support vector machine \emph{LinearSVC} to classify apps, a thorough set of static features extracted from Android apps that spans all app components, permissions, URL's, etc., and the \texttt{drebin} labeling strategy. 
Using an implementation of \emph{Drebin}'s feature extraction algorithm, we extracted a total of 71,260 features from apps in the \emph{AndroZoo}, \emph{Hand-Labeled}, \emph{Hand-Labeled 2019} datasets. 
In addition to \emph{Drebin}, we use the following classifiers: \emph{\gls{knn}} ~\cite{sanz2012automatic}, \emph{\gls{rf}} ~\cite{sanz2013puma}, \emph{\gls{svm}} ~\cite{arp2014drebin}, and \emph{\gls{gnb}}\footnote{Gaussian naive Bayes classifiers assume that features have a Gaussian distribution. We argue that the static features we extract from the apps indeed follow such distribution. For example, while a small number of apps request either a very small or a considerable amount of requests, the majority of apps request an adequate amount (e.g., in the lower tens).} ~\cite{sanz2013puma}. 
Given that the \gls{knn} and \gls{rf} classifiers can have different values for their hyperparameters, we used the technique of grid search to identify the classifiers that yielded the best validation accuracies and used them as representatives of those classifiers. 
We also varied the values of the primary hyperparameters of the \gls{knn} and \gls{rf} classifiers as follows; we varied the number of nearest neighbors to consider by the \gls{knn} classifier to $K=\lbrace 11,26,51,101\rbrace$ and the number of decisions trees in the random forest to $\lbrace 25,50,75,100\rbrace$. 
Consequently, we refer to these to classifiers as \gls{knn} and \gls{rf}. 
To train these classifiers, we statically extracted numerical features from the \gls{apk} archives of apps in the \emph{AndroZoo}, which depict information about the apps' components ~\cite{sato2013detecting,sanz2013puma}, the permissions they request ~\cite{arp2014drebin,wu2012droidmat}, the \gls{api} calls found in their codebases ~\cite{sachdeva2018android,zhou2013fast}, and the compilers used to compile them ~\cite{stazzere2016detecting}.  
  
The labeling strategies we consider in this experiment are the conventional threshold-based strategies of \texttt{vt$\geq$1}, \texttt{vt$\geq$4}, \texttt{vt$\geq$10}, \texttt{vt$\geq$50\%}, and \texttt{drebin}, threshold-based labeling strategies that use threshold brute-forced using at each point in time, threshold-based labeling strategies that use the best threshold at each point in time, and \Maat{}'s \gls{ml}-based labeling strategies that had the highest \gls{mcc} scores in the previous experiment, namely \texttt{Naive GS} and \texttt{Naive Sel GS}. 
In assessing the performance of different \gls{ml}-based detection methods, we are \textbf{not} concerned with absolute values that indicate the quality of the classifier and the features it is trained with.
Instead, we are interested in their performance with respect to one another. 
Given that the main difference between such classifiers is that their training feature vectors were labeled using different labeling strategies, this experiment is concerned with verifying the hypothesis of \emph{more accurate labeling leads to better detection}. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.47\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_Drebin_Hand-Labeled.pgf}}
		\caption{\emph{Hand-Labeled}}
		\label{fig:detection_drebin_hand-labeled}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_Drebin_Hand-Labeled2019.pgf}}
		\caption{\emph{Hand-Labeled 2019}}
		\label{fig:detection_drebin_hand-labeled2019}
	\end{subfigure}
	\caption{The \gls{mcc} scores achieved by the \emph{Drebin} classifiers labeled using different threshold-/\gls{ml}-based labeling strategies against the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} dataset between July 5$^{th}$, 2019 and \futureDate{}.}
	\label{fig:detection_drebin}
\end{figure}

In \autoref{fig:detection_drebin} we plot the classification performance of different \emph{Drebin} classifiers against apps in the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets in terms of \gls{mcc} score.
The feature vectors used to train each of those classifiers have been labeled using a different labeling strategy. 
Given that the performances of different classifiers are intertwined, we tabulate their \gls{mcc} scores in \autoref{tab:detection_drebin} for better readability. 
Studying these performances, we made the following observations. 

The first observation we made was that the performance of \emph{Drebin} classifiers is better on the \emph{Hand-Labeled 2019} dataset than on the older \emph{Hand-Labeled} dataset. 
The reason behind this is that apps in the \emph{AndroZoo} dataset were developed between 2018 and 2019. 
So, features extracted from these apps are expected to be similar to apps in the \emph{Hand-Labeled 2019} dataset than to those in the \emph{Hand-Labeled} dataset, especially since the \emph{Drebin} feature set is designed to identify similarity in the components and features utilized by the Android apps in the training dataset.
This proximity in feature space helps \emph{Drebin}'s \gls{svc} classifier identify patterns shared by malicious and benign apps better. 

\begin{table}[]
\centering
\caption{Detailed view of the \gls{mcc} scores achieved by the \emph{Drebin} classifiers labeled using different threshold-/\gls{ml}-based labeling strategies against the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} dataset between July 5$^{th}$, 2019 and \futureDate{}.}
\label{tab:detection_drebin}
\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}|c|cccccccccc|@{}}
\toprule
\backslashbox{Labeling Strategy}{Scan Date} & \rotatebox[origin=c]{90}{ 2019-07-05 } & \rotatebox[origin=c]{90}{ 2019-07-19 } & \rotatebox[origin=c]{90}{ 2019-08-02 } & \rotatebox[origin=c]{90}{ 2019-08-16 } & \rotatebox[origin=c]{90}{ 2019-08-30 } & \rotatebox[origin=c]{90}{ 2019-09-13 } & \rotatebox[origin=c]{90}{ 2019-09-27 } & \rotatebox[origin=c]{90}{ 2019-10-11 } & \rotatebox[origin=c]{90}{ 2019-10-25 } & \rotatebox[origin=c]{90}{ 2019-11-08 } \\ \hline
\multicolumn{11}{c}{\cellcolor[HTML]{C0C0C0}\textbf{\emph{Hand-Labeled}}} \\ \hline
Brute-forced Thresholds & 0.00 & 0.00 & 0.00 & 0.18 & 0.24 & 0.18 & 0.00 & 0.00 & 0.00 & 0.18 \\ \hline
Best Thresholds & 0.28 & 0.34 & 0.43 & 0.44 & 0.38 & 0.24 & 0.22 & 0.50 & 0.56 & 0.50 \\ \hline
\texttt{vt$\geq$1} & 0.21 & 0.24 & 0.15 & 0.28 & 0.31 & 0.27 & 0.35 & 0.25 & 0.31 & 0.31 \\ \hline
\texttt{vt$\geq$4} & 0.26 & 0.22 & 0.32 & 0.43 & 0.38 & 0.24 & 0.22 & 0.24 & 0.39 & 0.36 \\ \hline
\texttt{vt$\geq$10} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ \hline
\texttt{vt$\geq$50\%} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ \hline
\texttt{drebin} & 0.00 & 0.08 & 0.08 & 0.00 & 0.08 & 0.08 & 0.28 & 0.00 & 0.15 & 0.05 \\ \hline
\texttt{Naive GS} 2018 & 0.59 & 0.41 & 0.53 & 0.55 & 0.61 & 0.48 & 0.51 & 0.36 & 0.55 & 0.55 \\ \hline
\texttt{Naive GS} 2019-04-12 & 0.27 & 0.29 & 0.39 & 0.25 & 0.20 & 0.30 & 0.38 & 0.33 & 0.49 & 0.26 \\ \hline
\texttt{Naive Sel GS} 2018 & 0.54 & 0.51 & 0.60 & 0.55 & 0.59 & 0.54 & 0.72 & 0.38 & 0.55 & 0.55 \\ \hline
\texttt{Naive Sel GS} 2019-04-12 & 0.50 & 0.47 & 0.48 & 0.47 & 0.53 & 0.52 & 0.48 & 0.43 & 0.58 & 0.47 \\ \hline
\multicolumn{11}{c}{\cellcolor[HTML]{C0C0C0}\textbf{\emph{Hand-Labeled 2019}}} \\ \hline
Brute-forced Thresholds & 0.30 & 0.00 & 0.30 & 0.19 & 0.33 & 0.33 & 0.30 & 0.27 & 0.53 & 0.43 \\ \hline
Best Thresholds & 0.73 & 0.67 & 0.73 & 0.80 & 0.67 & 0.65 & 0.70 & 0.66 & 0.73 & 0.76 \\ \hline
\texttt{vt$\geq$1} & 0.18 & 0.18 & 0.19 & 0.18 & 0.24 & 0.26 & 0.34 & 0.25 & 0.40 & 0.37 \\ \hline
\texttt{vt$\geq$4} & 0.73 & 0.66 & 0.80 & 0.73 & 0.76 & 0.70 & 0.73 & 0.78 & 0.80 & 0.73 \\ \hline
\texttt{vt$\geq$10} & 0.53 & 0.23 & 0.43 & 0.38 & 0.33 & 0.33 & 0.43 & 0.27 & 0.48 & 0.48 \\ \hline
\texttt{vt$\geq$50\%} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ \hline
\texttt{drebin} & 0.23 & 0.00 & 0.10 & 0.10 & 0.02 & 0.04 & 0.14 & 0.19 & 0.23 & 0.19 \\ \hline
\texttt{Naive GS} 2018 & 0.84 & 0.76 & 0.73 & 0.63 & 0.80 & 0.76 & 0.70 & 0.67 & 0.80 & 0.78 \\ \hline
\texttt{Naive GS} 2019-04-12 & 0.84 & 0.78 & 0.80 & 0.78 & 0.78 & 0.84 & 0.71 & 0.67 & 0.80 & 0.82 \\ \hline
\texttt{Naive Sel GS} 2018 & 0.71 & 0.69 & 0.63 & 0.69 & 0.71 & 0.69 & 0.69 & 0.71 & 0.69 & 0.62 \\ \hline
\texttt{Naive Sel GS} 2019-04-12 & 0.76 & 0.80 & 0.80 & 0.76 & 0.76 & 0.76 & 0.73 & 0.80 & 0.73 & 0.84 \\ \bottomrule
\end{tabular}}
\end{table}

Secondly, we found that using best threshold at each point on time along with \Maat{}'s \gls{ml}-based labeling strategies usually helps the \emph{Drebin} classifier achieve better \gls{mcc} scores than threshold-based labeling strategies that use fixed thresholds over time (e.g., \texttt{vt$\geq$1}, \texttt{vt$\geq$10}, and \texttt{vt$\geq$50\%}). 
Moreover, the average \gls{mcc} scores of \emph{Drebin} classifiers labeled using \Maat{}'s \gls{ml}-based labeling strategies is higher than that of classifiers labeled using the best thresholds at each scan date. 
This observation coincides with our hypothesis that accurate labeling strategies, by and large, contribute to training more effective \gls{ml}-based detection methods. 
However, we noticed a number of exceptions that contradict this hypothesis. 
For example, the \texttt{Naive GS} \gls{ml}-based labeling strategies trained in \earliestDate{} and the \texttt{Naive GS} strategies trained on April 12$^{th}$, 2019 had almost the same labeling accuracy against apps in the \emph{Hand-Labeled} dataset. %(see \autoref{fig:mccs_over_time_2}).  
Despite this similarity, the \emph{Drebin} classifiers labeled using the latter strategy noticeably underperforms in comparison to the former one. 
This behavior switches on the \emph{Hand-Labeled 2019} dataset: the performance of \emph{Drebin} classifiers labeled using \texttt{Naive GS} 2018 almost mimics that of those labeled using \texttt{Naive GS} trained on April 12$^{th}$, 2019, despite the former being less able to label apps in this dataset accurately. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.47\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_KNN_Hand-Labeled.pgf}}
		\caption{\gls{knn} with \emph{Hand-Labeled}}
		\label{fig:detection_knn_hand-labeled}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_KNN_Hand-Labeled2019.pgf}}
		\caption{\gls{knn} with \emph{Hand-Labeled 2019}}
		\label{fig:detection_knn_hand-labeled2019}
	\end{subfigure}
	
		\begin{subfigure}[b]{0.47\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_RF_Hand-Labeled.pgf}}
		\caption{\gls{rf} with \emph{Hand-Labeled}}
		\label{fig:detection_rf_hand-labeled}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_RF_Hand-Labeled2019.pgf}}
		\caption{\gls{rf} with \emph{Hand-Labeled 2019}}
		\label{fig:detection_rf_hand-labeled2019}
	\end{subfigure}
	
		\begin{subfigure}[b]{0.47\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_GNB_Hand-Labeled.pgf}}
		\caption{\gls{gnb} with \emph{Hand-Labeled}}
		\label{fig:detection_gnb_hand-labeled}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\scalebox{0.42}{\input{figures/Line_Detection_GNB_Hand-Labeled2019.pgf}}
		\caption{\gls{gnb} with \emph{Hand-Labeled 2019}}
		\label{fig:detection_gnb_hand-labeled2019}
	\end{subfigure}
	
	\caption{The \gls{mcc} scores achieved by the \gls{knn}, \gls{rf}, and \gls{gnb} classifiers labeled using different threshold-/\gls{ml}-based labeling strategies against the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} dataset between July 5$^{th}$, 2019 and \futureDate{}.}
	\label{fig:detection_others}
\end{figure}

The third observation depicts another counter-example to the hypothesis that related accurate labeling to effective detection. 
Although it falls within the ranges of best thresholds identified at each scan date, using a threshold of four \VT{} scanners to label the \emph{Drebin} classifier (i.e., using \texttt{vt$\geq$4}), yields scores that do not mimic the performance of the \emph{Drebin} classifiers using the current best thresholds. 
For example, while using any threshold between three and six on July 5$^{th}$, 2019 resulted in the same \gls{mcc} scores against apps in the \emph{Hand-Labeled} dataset, on the same scan date and using the same test datasets, training a \emph{Drebin} classifier using a threshold of three scanners yields a different \gls{mcc} score than a classifier using a threshold of four scanners, namely 0.28 and 0.26, respectively. 

In general, we noticed that \gls{mcc} score of each \emph{Drebin} classifier differs depending on the utilized labeling strategy and the scan date of the \VT{} scan reports this strategy uses to label apps. 
In addition to these two factors, we noticed that the utilized classifier also impacts these scores. 
\autoref{fig:detection_others} shows the \gls{mcc} scores achieved by the \gls{knn}, \gls{rf}, and \gls{gnb} classifiers against the same test datasets using the same labeling strategies. 
Similar to the \emph{Drebin} classifier, the \gls{mcc} scores achieved by these three classifiers show that \Maat{}'s \gls{ml}-based labeling strategies contribute to training more effective detection methods than their threshold-based counterparts, in spite of using a different set of features to represent the apps in the training and test datasets. 
However, unlike the \emph{Drebin} classifier, the \gls{mcc} scores of the \gls{knn}, \gls{rf}, and \gls{gnb} classifiers seem to be stable across different scan dates, especially on the \emph{Hand-Labeled 2019} dataset. 
The values of these scores seem to differ from one classifier to another. 
On the \emph{Hand-Labeled 2019} dataset, for instance, the average \gls{mcc} scores of the \gls{knn}, \gls{rf}, and \gls{gnb} classifiers were 0.64, 0.89, and 0.43, respectively. 
So, it seems that the features used to represent apps in the training dataset and the type of \gls{ml} classifier also impact the performance of a detection method. 

To sum up, we found that accurately labeling apps based on their \VT{} scan reports does not guarantee training more effective detection methods.
Other factors, such as the utilized feature set and the date on which the training and test apps were scanned by \VT{} also impact the effectiveness of such methods. 
%This raises the question: what role does accurate labeling strategy play in the process of Android malware detection?
%In order to objectively assess the role of accurate labeling in the malware detection process, we to understand the upper bounds of accurate labeling and the limitations that it cannot overcome. 
%Consider the illustration in \autoref{fig:zeroday_explanation}. 
%Assume that we have a set of Android malicious (circles) and benign (triangles) apps that are represented using a two-dimensional feature set, as seen in \autoref{fig:zeroday_explanation1}. 
%Using the \VT{} scan reports of those apps, we can label those apps using different labeling strategies. 
%In \autoref{fig:zeroday_explanation2}, for example, we use \texttt{vt$\geq$1} to label apps into malicious (red) and benign (green). 
%The labels assigned to the apps are going to impact the decision boundary a detection methods (e.g., \emph{\gls{svm}}), will attempt to draw to separate apps into malicious and benign. 
%The more accurate a labeling strategy is, the more precise a detection method can draw a decision boundary between malicious and benign apps, which will impact the labels given to out-of-sample apps, including zero-day malware depicted here as an orange diamond. 
%For example, the labeling strategy used in \autoref{fig:zeroday_explanation2} label the apps in manner that would put the orange diamond on the side of malicious apps, while using a labeling strategy that is more biased towards labeling apps as benign (e.g., \texttt{vt$\geq$50\%}), the diamond will more likely be on the side of benign apps, as seen in \autoref{fig:zeroday_explanation3}. 
%
%In this hypothetical scenario, \texttt{Naive (Sel) GS} labels apps as malicious and benign more accurately than \texttt{vt$\geq$1} and \texttt{vt$\geq$50\%}. 
%However, this does not guarantee that the zero-day app is indeed malicious. 
%Adopting a different feature set or a high-dimensional feature space may position the app's representation on a different side of the learned classification boundary. 
%So, labeling strategies enable detection methods to be trained using more accurate labels and, in theory, be more effective. 
%This does not impact the detection methods' abilities to detect apps far from what it has seen before (e.g., because they are newer ~\cite{pendlebury2019}).
%
%\begin{figure}
%\centering
%\begin{subfigure}[b]{0.24\textwidth}
%	\centering
%    \includegraphics[scale=0.75]{figures/zeroday_explanation1}
%    \caption{Unlabeled}
%    \label{fig:zeroday_explanation1}
%\end{subfigure}
%\begin{subfigure}[b]{0.24\textwidth}
%	\centering
%    \includegraphics[scale=0.75]{figures/zeroday_explanation4}
%    \caption{\texttt{vt$\geq$1}}
%    \label{fig:zeroday_explanation2}
%\end{subfigure}
%\begin{subfigure}[b]{0.24\textwidth}
%	\centering
%    \includegraphics[scale=0.75]{figures/zeroday_explanation3}
%    \caption{\texttt{vt$\geq$50\%}}
%    \label{fig:zeroday_explanation3}
%\end{subfigure}
%\begin{subfigure}[b]{0.24\textwidth}
%	\centering
%    \includegraphics[scale=0.75]{figures/zeroday_explanation2}
%    \caption{\texttt{Naive (Sel) GS}}
%    \label{fig:zeroday_explanation4}
%\end{subfigure}
%\caption[An illustration of the processes of labeling Android apps and using the labeled apps to train detection methods]{An illustration of the processes of labeling Android apps and using the labeled apps to train detection methods. Uncolored circles, triangles, and diamond depict malicious, benign, and unknown (zero-day) apps. Shapes colored in red indicate a malicious label, shapes colored in green indicate a benign label, and shapes colored in orange indicate an unknown label.}
%\label{fig:zeroday_explanation}
%\end{figure}
%
%In \autoref{fig:androzoo_visualization} we visualize apps in the \emph{AndroZoo} dataset in two-dimensional space using the \gls{pca} projection of static features extracted from their \gls{apk} archives (see appendix \ref{appendix:static_features}), viz.\ the features we used to train and validate the \gls{knn}, \gls{rf}, and \gls{gnb} classifiers. 
%As an example of zero-day apps, we use apps in the \emph{Homegrown} dataset, which are all malicious because we consciously implemented them to deliver malicious functionalities. 
%The \gls{pca} projection is an approximation of the relationships between apps in lower-dimensional spaces and, thus, serves the purpose of our explanation. 
%In \autoref{fig:androzoo_visualization_vt1}, the bias of \texttt{vt$\geq$1} towards labeling apps as malicious and that of \texttt{vt$\geq$50\%} towards labeling apps as benign are noticeable. 
%Using the \texttt{vt$\geq$1} labeling strategy results in labeling the majority of apps in the \emph{AndroZoo} dataset as malicious. 
%Recall that apps in this were randomly downloaded from the \emph{AndroZoo} platform without bias towards malicious or benign apps. 
%Consequently, the percentage of malicious apps in either dataset should be around 10\% rather than a majority ~\cite{pendlebury2018enabling}. 
%The imbalance in the number of malicious and benign apps caused by using \texttt{vt$\geq$1} instigates \gls{ml} classifiers to favor classifying apps as malicious, which does not have noticeable negative impacts on the learning error, as discussed in \autoref{sec:AndroidDetection_MLBased}. 
%Intuitively, \gls{ml} classifiers biased towards malicious apps are expected to perform well on test datasets exclusively comprising malicious apps. 
%
%To give an example of such bias, consider the \gls{knn} classifiers trained using apps in the \emph{AndroZoo} dataset, and labeled using the \texttt{vt$\geq$1} labeling strategy. 
%These classifiers deem apps as malicious if the nearest ($K$) neighbors in the training dataset are malicious. 
%Under the \texttt{vt$\geq$1} labeling strategy, it is likely that such ($K$) neighbors are deemed to be malicious, effectively causing the \gls{knn} classifiers to deem test apps as such. 
%For example, in \autoref{fig:androzoo_visualization_vt1}, the light blue diamond falling with the ($x_1$,$x_2$) coordinates ($-2000\geq x_1\leq 0$, $2000\geq x_2\leq 3000$) depicting an malicious app from the \emph{Homegrown} dataset appears to be surrounded by more malicious apps (i.e., red circles), than benign ones.
%Using \texttt{vt$\geq$50\%} yields the exact opposite behavior and classification performance to using \texttt{vt$\geq$1}. 
%That is, the majority of training apps, as seen in \autoref{fig:androzoo_visualization_vt50p}, are labeled as benign (i.e., green triangles), making the recognition of the malignancy of the \emph{Homegrown} app in question highly unlikely. 
%
%%\begin{sidewaysfigure}
%\begin{figure*}
%\centering
%\begin{subfigure}[b]{0.44\textwidth}
%	\centering
%    \includegraphics[scale=0.42]{figures/Visualization_androzoo_2019_vt1}
%    \caption{\emph{AndroZoo} and \texttt{vt$\geq$1}}
%    \label{fig:androzoo_visualization_vt1}
%\end{subfigure}
%\begin{subfigure}[b]{0.44\textwidth}
%	\centering
%    \includegraphics[scale=0.42]{figures/Visualization_androzoo_2019_vt50p}
%    \caption{\emph{AndroZoo} and \texttt{vt$\geq$50\%}}
%    \label{fig:androzoo_visualization_vt50p}
%\end{subfigure}
%\begin{subfigure}[b]{0.44\textwidth}
%	\centering
%    \includegraphics[scale=0.42]{figures/Visualization_androzoo_2019_vt4}
%    \caption{\emph{AndroZoo} and \texttt{vt$\geq$4}}
%    \label{fig:androzoo_visualization_vt4}
%\end{subfigure}
%\begin{subfigure}[b]{0.44\textwidth}
%	\centering
%    \includegraphics[scale=0.42]{figures/Visualization_androzoo_2019_naive_sel_gs}
%    \caption{\emph{AndroZoo} and \texttt{Naive Sel GS}}
%    \label{fig:androzoo_visualization_naive_sel_gs}
%\end{subfigure}
%\caption{A two-dimensional, \gls{pca}-generated visualization of apps in the \emph{AndroZoo} and \emph{Homegrown} datasets using static features (see appendix \ref{appendix:static_features}) extracted from their \gls{apk} archives. The apps are labeled as malicious and benign based on their \VT{} scan reports downloaded on \futureDate{} and using the labeling strategies \texttt{vt$\geq$1}, \texttt{vt$\geq$50\%}, \texttt{vt$\geq$4}, and \texttt{Naive Sel GS}.}
%\label{fig:androzoo_visualization}
%\end{figure*}
%
%As for using more balanced labeling strategies, namely \texttt{vt$\geq$4} and \texttt{Naive Sel GS}, the visualizations in \autoref{fig:androzoo_visualization_vt4} and\autoref{fig:androzoo_visualization_naive_sel_gs}, the percentages of malicious and benign apps in the training datasets appear to reflect the percentages expected and recommended by the research community. 
%However, the performance of \gls{ml}-based detection methods labeled using such strategies is subject to the proximity of apps in the \emph{Homegrown} dataset to malicious or benign apps rather than their labeling accuracy.  
%In the case of \gls{knn} classifiers, such proximity is defined in terms of the distances between the apps' feature vectors (e.g., Euclidean distance). 
%So, if the majority of the feature vectors neighboring the vector representing a \emph{Homegrown} app correspond to malicious apps, the \emph{Homegrown} app will be correctly deemed as malicious. 
%Otherwise, the feature vector and its corresponding app will be classified as benign. 
%For example, in \autoref{fig:androzoo_visualization_vt4} and \autoref{fig:androzoo_visualization_naive_sel_gs}, the \emph{Homegrown} app whose ($x_2$) value is between 2000 and 3000 is surrounded by more malicious apps than benign, whereas the app whose ($x_1$) and ($x_2$) values are both at zero is surrounded by more benign apps than malicious. 
%Respectively, the two apps are expected to--and were actually--classified by \gls{knn} classifiers labeled using \texttt{vt$\geq$4} and \texttt{Naive Sel GS} as malicious and benign. 
%In general, the closer the feature vector of a \emph{Homegrown} app is to other malicious apps in the training dataset, the more likely they are to be labeled as malicious. 
%
%So, what does that say about the performance of \gls{ml}-based detection methods against out-of-sample Android apps, including zero-day malware? 
%The ability of a \gls{ml} classifier to recognize the malignancy of a feature vector and its corresponding app hinges on the ability of the features extracted from the training and test apps' \gls{apk} archives to cluster malicious and benign apps together. 
%This facilitates devising a decision boundary (e.g., in the case of \gls{svm}), or a model that separates both classes of apps and increases the likelihood of assigning an out-of-sample app to its correct class. 
%Not only does this apply for zero-day malware, but it also applies to all test apps. 
%The notion of zero-day, as we argued earlier in this chapter, is used by human analysts and researchers to refer to newly-developed malicious Android apps that evade detection by automated detection methods (e.g., antiviral software). 
%However, automated detection methods, including \gls{ml}-based ones, do not differentiate between out-of-sample malicious apps, whether they are newly-developed or clones of older ones. 
%\gls{ml}-based detection methods will successfully label an out-of-sample app as malicious if it shares characteristics with malicious apps in its training dataset that manifests in the features extracted from the app's \gls{apk} archive. 
%
%The role that labeling plays in the process of learning this decision boundary or model is fundamental. 
%Inaccurate labeling strategies (e.g., ones that are biased towards one class) force \gls{ml} classifiers to learn characteristics about a class of apps, that are not inherent in this class. 
%For example, just because they are inaccurately labeled as benign, a classifier might learn that benign Android apps often request more permissions than they need, which is usually a characteristic of malicious apps ~\cite{li2017understanding,zhou2012dissecting}. 
%Learning false characteristics or features ultimately leads to devising decision boundaries and models that inaccurately classify test apps. 
%In other words, accurate labeling is a prerequisite to accurate learning and classification but cannot always guarantee it. 

==> backup/correctness.tex <==
\section{Correctness of \texttt{VirusTotal} Scanners}
\label{sec:correctness}
As part of extracting engineered features to train \Maat{}'s \gls{ml}-based labeling strategies, in this section, we attempt to identify the \texttt{VirusTotal} scanners that are consistently more correct than others at labeling Android apps.  
That is, we attempt to address the research question:

\begin{tcolorbox}[colback=white]%[title=\textbf{RQ3},colback=white]
	\footnotesize
	\textbf{RQ1} \RQone
\end{tcolorbox}

For this task, we consider the \emph{AMD} dataset instead of the \emph{AMD+GPlay} for the following reasons.
First, all the apps in the \emph{GPlay} dataset have \emph{positives} of zero (i.e., all scanners labeled them correctly as benign). 
So, calculating the correctness of scanners using apps in the \emph{GPlay} dataset does not add useful information about the correctness of scanners. 
Second, using benign apps, it is difficult to assess the competence of a scanner. 
That is, it is difficult to assess whether an app has been analyzed by a scanner and was consciously deemed as benign, whether the app was never seen and analyzed by the scanner and gets assigned the label benign, or whether the scanner follows the verdicts of other, perhaps more established or renowned, scanners. 
Given that benign apps comprise the majority of Android apps ~\cite{pendlebury2018enabling}, defaulting to a label of benign is more likely to be the correct one. 
So, with benign apps, the inaccuracy of some antiviral scanners remains unnoticed as they appear to be scanners that correctly labeled an app. 
Such inaccuracy is revealed upon introducing malicious apps to the dataset, which must be analyzed before deeming them as malicious, primarily since antiviral scanners are known to be cautious in deeming apps as such ~\cite{menn2015reuters}. 
Third, since we have information about the malware types and families that the apps in the \emph{AMD} dataset belong to, we can gain insights about the malware types that \texttt{VirusTotal} scanners excel at detecting.
Lastly, we consider the \emph{AMD} dataset because human analysts were involved in generating the ground truth labels for apps in the dataset (i.e., as discussed in \autoref{subsec:preliminaries_datasets}), which we assume makes such a ground truth more credible. 

% from Maat.mining import correctness
% correctness.getCorrectnessByType(datasetDir, vtReportsDir, groundTruth, hashToTypeMapping) # Only hash to type, not to type and family
\bgroup
\def\arraystretch{1.0}
\begin{table*}[]
%\begin{sidewaystable}
\centering
\caption{The change in the correctness rates of the \emph{Drebin} \texttt{VirusTotal} scanners on apps in the \emph{AMD} dataset between \earliestDate{} and \latestDate{}, grouped by malware type.}
\label{tab:correctness}
%\small
\footnotesize
\resizebox{\textwidth}{!}{
%\begin{tabular}{@{}|c|c|c|c|c|c|c|c|c|c|@{}}
\begin{tabular}{@{}|c|cccccccccc|@{}}
\toprule
\backslashbox{Malware Types}{\emph{Drebin} Scanners} & \texttt{AVG} & \texttt{Avira} & \texttt{BitDefender} & \texttt{ClamAV} & \texttt{ESET} & \texttt{F-Secure} & \texttt{Kaspersky} & \texttt{McAfee} & \texttt{Panda} & \texttt{Sophos} \\ \hline

\texttt{Adware} & \textcolor{ACMRed}{\emph{0.01}$\rightarrow$\emph{0.01}} & 0.91$\nearrow$0.99 & 0.45$\searrow$0.0 & 0.10$\rightarrow$0.10 & 0.98$\nearrow$0.99 & 0.53$\nearrow$0.99 & \textcolor{ACMRed}{\emph{0.26}$\nearrow$\emph{0.33}} & 0.95$\nearrow$0.99 & \textcolor{ACMOrange}{\underline{0.0}$\rightarrow$\underline{0.0}} & 0.92$\nearrow$0.95 \\ \hline

\texttt{Backdoor} & 0.92$\nearrow$0.93 & 0.96$\nearrow$0.99 & 0.97$\searrow$0.1 & 0.61$\rightarrow$0.61 & 0.99$\nearrow$1.0 & 0.89$\nearrow$0.99 & 0.98$\rightarrow$0.98 & 0.99$\rightarrow$0.99 & \textcolor{ACMOrange}{\underline{0.01}$\rightarrow$\underline{0.01}} & 0.98$\nearrow$0.99 \\ \hline

\texttt{HackerTool} & 0.99$\nearrow$1.0 & 0.99$\rightarrow$0.99 &\textcolor{ACMGreen}{\textbf{0.99$\searrow$0.90}} & \textcolor{ACMGreen}{\textbf{0.91}$\rightarrow$\textbf{0.91}} & \textcolor{ACMRed}{\emph{0.81}$\rightarrow$\emph{0.81}} & 0.89$\nearrow$1.0 & \textcolor{ACMRed}{\emph{0.75}$\rightarrow$\emph{0.75}} & 0.99$\rightarrow$0.99 & \textcolor{ACMOrange}{\underline{0.32}$\rightarrow$\underline{0.32}} & 0.99$\rightarrow$0.99\\ \hline

\texttt{Ransom} & 0.98$\nearrow$0.99 & 0.99$\rightarrow$1.0 & 0.98$\searrow$0.0 & 0.05$\nearrow$0.06 & 0.99$\nearrow$1.0 & 0.89$\nearrow$1.0 & 0.99$\nearrow$1.0 & 0.99$\nearrow$1.0 & \textcolor{ACMOrange}{\underline{0.0}$\rightarrow$\underline{0.0}} & 0.99$\rightarrow$0.99 \\ \hline

\texttt{Trojan} & 0.84$\rightarrow$0.84 & 0.96$\nearrow$1.0 & 0.88$\searrow$0.01 & 0.10$\searrow$0.07 & 0.96$\rightarrow$0.96 & 0.75$\nearrow$1.0 & 0.88$\rightarrow$0.88 & 0.99$\nearrow$1.0 & \textcolor{ACMOrange}{\underline{0.0}$\rightarrow$\underline{0.0}} & 0.97$\nearrow$0.98 \\ \hline

\texttt{Trojan-Banker} & 0.98$\nearrow$0.99 & 0.99$\rightarrow$0.99 & 0.99$\searrow$0.0 & 0.09$\rightarrow$0.09 & 0.99$\nearrow$1.0 & 0.92$\nearrow$1.0 & 0.99$\rightarrow$0.99 & 0.99$\nearrow$1.0 & \textcolor{ACMOrange}{\underline{0.0}$\rightarrow$\underline{0.0}} & 0.99$\nearrow$1.0 \\ \hline

\texttt{Trojan-Clicker} & 0.96$\nearrow$1.0 & 1.0$\rightarrow$1.0 & 1.0$\searrow$0.0 & 0.32$\rightarrow$0.32 & 1.0$\rightarrow$1.0 & 0.87$\nearrow$1.0 & 0.96$\searrow$0.90 & 1.0$\rightarrow$1.0 & \textcolor{ACMOrange}{\underline{0.0}$\rightarrow$\underline{0.0}} & 1.0$\rightarrow$1.0 \\ \hline

\texttt{Trojan-Dropper} & 0.98$\nearrow$0.99 & 0.96$\nearrow$0.99 & 0.96$\searrow$0.03 & 0.10$\nearrow$0.11 & 0.97$\nearrow$0.99 & 0.80$\nearrow$0.99 & 0.97$\nearrow$0.98 & 0.98$\nearrow$1.0 & \textcolor{ACMOrange}{\underline{0.02}$\rightarrow$\underline{0.0}} & 0.97$\nearrow$0.99 \\ \hline

\texttt{Trojan-SMS} & 0.88$\rightarrow$0.88 & 0.99$\nearrow$1.0 & 0.98$\searrow$0.0 & 0.24$\searrow$0.15 & 0.99$\rightarrow$0.99 & 0.88$\nearrow$1.0 & 0.98$\nearrow$0.99 & 0.99$\nearrow$1.0 & \textcolor{ACMOrange}{\underline{0.0}$\rightarrow$\underline{0.0}} & 0.99$\rightarrow$0.99 \\ \hline

\texttt{Trojan-Spy} & 0.05$\nearrow$0.87 & 0.99$\nearrow$1.0 & 1.0$\searrow$0.0 & 0.01$\rightarrow$0.01 & 0.99$\nearrow$1.0 & 0.61$\rightarrow$1.0 & 0.99$\rightarrow$0.99 & 0.99$\nearrow$1.0 & \textcolor{ACMOrange}{\underline{0.0}$\rightarrow$\underline{0.0}} & 0.99$\rightarrow$0.99 \\ \hline

Overall Correctness & 0.34$\nearrow$0.40 & 0.\textbf{94}$\nearrow$\textbf{1.0} & 0.68$\searrow$0.02 & 0.15$\searrow$0.13 & \textbf{0.99}$\nearrow$\textbf{1.0} & 0.66$\nearrow$\textbf{0.99} & 0.57$\nearrow$0.61 & \textbf{0.97}$\nearrow$\textbf{1.0} & \textcolor{ACMOrange}{\underline{0.01}$\rightarrow$\underline{0.01}} & \textbf{0.95}$\nearrow$\textbf{0.97} \\ \bottomrule
\end{tabular}}
\end{table*}
%\end{sidewaystable}
\egroup

As for the definition of \emph{correctness}, we rely on Mohaisen et al.'s definition: For a given dataset, the correctness of an antiviral scanner is the
number of correct detections normalized by the size of the dataset \cite{mohaisen2014av}. 
So, for each \texttt{VirusTotal} scanner, we calculate the number of apps in the \emph{AMD+GPlay} dataset it managed to correctly label as malicious, and divide that number by the size of the dataset or by the number of apps belonging to a particular malware type upon focusing on the correctness of scanners per malware type.
 
Given that \texttt{VirusTotal} comprises around 60 scanners, we can only display and discuss the results of a subset of scanners, viz.\ ones utilized by Arp et al.\ in \cite{arp2014drebin} to label apps in the \emph{Drebin} dataset.  
These scanners are \texttt{AntiVir}\footnote{\texttt{AntiVir} refers to the antiviral scanner developed by \texttt{Avira}, which is the name that \texttt{VirusTotal} uses for this scanner now.}, \texttt{AVG}, \texttt{BitDefender}, \texttt{ClamAV}, \texttt{ESET}, \texttt{F-Secure}, \texttt{Kaspersky}, \texttt{McAfee}, \texttt{Panda}, and \texttt{Sophos}. 
We refer to this group of scanners as the \emph{Drebin} scanners.

The results in \autoref{tab:correctness} show the evolution of the overall correctness of the \emph{Drebin} scanners on the \emph{AMD} dataset according to \texttt{VirusTotal} scan reports downloaded on \earliestDate{} and on \latestDate{} along with the correctness per malware type. 
As per the overall correctness rates, it is evident that some scanners are more correct than others (e.g., \texttt{ESET}, \texttt{McAfee}, and \texttt{Sophos}). 
The following observations can be made upon considering the correctness rates per malware type. 
Firstly, scanners that have decent overall correctness usually score high correctness rates on all malware types. 
As for the correctness rates per malware type, on the one hand, some scanners achieve high correctness rates on the majority of malware types yet struggle with others. 
For example, \texttt{AVG} and \texttt{Kaspersky} appear to struggle with apps belonging to the \texttt{Adware} malware type (emphasized red). 
On the other hand, some scanners excel against particular malware types, such as \texttt{BitDefender} and \texttt{ClamAV}, which continue to correctly detect the \texttt{HackerTool} malware type.
As seen in emboldened green, \texttt{BitDefender} and \texttt{ClamAV} appear to score decent correctness rates on the \texttt{HackerTool} malware type, whilst struggling with all other types.
Lastly, some scanners, such as \texttt{Panda}, appear to struggle on all malware types, even though some apps in the \emph{AMD} dataset are as old as 2010 \cite{wei2017deep}. 

% from Maat.mining import correctness
% correctness.getCorrectnessOverTime(datasetDir, vtReportsDirs, groundTruth, generateLinePlot, plotScanners)
% correctness.getMostCorrectScannersOverTime(datasetDir, vtReportsDirs, groundTruth, averageCorrectness=0.9, generateLinePlots, plotScanners)
\begin{figure}
\centering
\scalebox{0.5}{\input{figures/Line_correctness_10_scanners.pgf}}
\caption{The overall correctness rates of the \emph{Drebin} scanners on apps in the \emph{AMD} dataset between \earliestDate{} and \latestDate{}.}
\label{fig:correctness_over_time}
\end{figure}

In \autoref{fig:correctness_over_time}, we measure the overall correctness of the \emph{Drebin} scanners between \earliestDate{} and \latestDate{}. 
Similar to the results in \autoref{tab:correctness}, some \texttt{VirusTotal} scanners are more correct than others over time. 
Moreover, it appears that--within the given time period--some of the \emph{Drebin} scanners have had stable correctness rates since \earliestDate{}, such as \texttt{Kaspersky}, \texttt{McAfee}, and \texttt{Panda}. 
However, we noticed that the correctness of \texttt{F-Secure} noticeably oscillates on a frequent basis. 
For example, the overall correctness of the scanner steeply dropped from above 0.90 on June 7$^{th}$, 2019 to around 0.70 on June 21$^{st}$, 2019 only to increase to 0.90 two weeks later on \interDate{}. 
We also noticed that the correctness of \texttt{BitDefender} significantly dropped between \earliestDate{} and April 12$^{th}$, 2019, and remained at 0.02.  
Despite this mediocre performance reported by \texttt{VirusTotal}, \texttt{BitDefender} continues to be given good reviews by users on the Google Play marketplace and, more importantly, on platforms that assess the effectiveness of antiviral software such as \emph{AV-Test} ~\cite{avtest2019}. 
We hypothesize that this performance discrepancy might be due to \texttt{VirusTotal} using different versions of scanners, especially since it states that the scanners it uses "\emph{may differ from commercial off-the-shelf products. The [antiviral software] company decides the particular settings with which the engine should run in VirusTotal}" ~\cite{virustotal2019}. 
We found that, as of September 2019, the version used by \texttt{VirusTotal}'s for \texttt{BitDefender} is 7.2, whereas the versions available on Google Play have codes between 3.3 and 3.6. 
The 7.2 version of \texttt{BitDefender} corresponds to a free edition version developed for Windows-based malware that targets older versions of Windows such as \texttt{Windows XP} ~\cite{pcmagazin2008bitdefender}. 

In this context, we hypothesized that using a recent, adequate version of \texttt{BitDefender} (i.e., one that is designed to detect Android malware), would yield a detection performance better than the version on \texttt{VirusTotal}. 
To verify this hypothesis, we downloaded and installed the latest version of the \texttt{BitDefender} scanner from the Google Play marketplace, installed it on an \gls{avd}, and used it to scan \href{https://github.com/tum-i22/Maat#bitdefender-and-panda-on-virustotal-versus-reality}{\underline{ten apps}} randomly sampled from the \emph{AMD} dataset. 
Unlike the results obtained from \texttt{VirusTotal} that the scanners are unable to detect any of those apps, we found that \texttt{BitDefender} detects 70\% of the sampled apps.
Similarly, albeit still being a low detection rate, the latest version of the \texttt{Panda} scanner detected 30\% of the sampled apps as opposed to the 0\% rate reported by \texttt{VirusTotal}.  
We performed the same measurement using the Google Play versions of the best-performing \emph{Drebin} scanners (e.g., \texttt{ESET-NOD32}), to investigate whether performance discrepancies occur in the case of scanners that perform well according to the \texttt{VirusTotal} scan reports. 
In this case, the performance of such scanners on the aforementioned ten apps matched the scan reports on \texttt{VirusTotal}.

The results above suggest that \texttt{VirusTotal} scan reports do not necessarily reflect the performance of scanners in the wild. 
While this does not impact our results and calculations of the best-performing scanners, it might undermine the usefulness of \texttt{VirusTotal} in labeling apps. 
From a research perspective, solely relying on \texttt{VirusTotal}'s scan reports might lead to publishing inaccurate results and false claims (e.g., that \texttt{BitDefender}'s detection capability is mediocre). 
In fact, \texttt{VirusTotal} seems to be aware of such a limitation and discourages researchers from comparing the performance of antiviral scanners: "\emph{\texttt{VirusTotal} should not be used to generate comparative metrics between different antivirus products. Antivirus engines can be sophisticated tools that have additional detection features that may not function within the VirusTotal scanning environment. Because of this, VirusTotal scan results are not intended to be used for the comparison of the effectiveness of antivirus products.}" ~\cite{virustotal2019maintaining}. 

%So, do some antiviral software companies believe that offering older versions on \texttt{VirusTotal} will encourage users to download their products instead of relying on the online version available on \texttt{VirusTotal}? 
%Do such companies enforce a fee on \texttt{VirusTotal} in order to use their new products, which the latter did not agree to?
Unfortunately, without access to the nature of the agreements between \texttt{VirusTotal} and antiviral software, it is not possible to identify the reasons behind utilizing older, inadequate versions to scan apps uploaded to the platform. 
Answering those questions is not in the scope of this paper and, in fact, impossible to answer on behalf of antiviral software companies. 
So, to address our research questions, we have to constrain our results to \texttt{VirusTotal}. 
According to the results of \texttt{VirusTotal}, we managed to identify an ensemble of scanners that are more correct than others over the time period between \earliestDate{} and \latestDate{}. 
To retrieve the list of scanners that are most correct, we focused on those that maintained an average of at least 0.90 (i.e., 90\%) overall correctness on the \emph{AMD} dataset between \earliestDate{} and \latestDate{}. 
We chose the number 0.90 to tolerate any fluctuations in the correctness rate that may occur, for example, due to changing policies on how to label ambiguous malware types, such as \texttt{Adware}, or the temporary use of inadequate versions of scanners. 
Using this criterion, we retrieved a list of \CorrectScannersCount{}, namely \texttt{Avira}, \texttt{CAT-QuickHeal}, \texttt{DrWeb}, \texttt{ESET-NOD32},  \texttt{Fortinet}, \texttt{Ikarus}, \texttt{MAX}, \texttt{McAfee}, \texttt{NANO-Antivirus}, \texttt{Sophos}, and \texttt{SymantecMobileInsight} that we utilize as part of the engineered features extracted from \texttt{VirusTotal} scan reports to train \Maat{}'s \gls{ml}-based labeling strategies. 
% Drebin: AVG, Avira (AntiVir), BitDefender, ClamAV, ESET-NOD32, F-Secure, Kaspersky, McAfee, Panda, Sophos
% Ours: Avira, CAT-QuickHeal, DrWeb, ESET-NOD32, Fortinet, Ikarus, MAX, McAfee, NANO-Antivirus, Sophos, SymantecMobileInsight

Although the number of \texttt{VirusTotal} scanners we found to be correct is similar to the number of the \emph{Drebin} scanners Arp et al.\ used in 2014 to label apps ~\cite{arp2014drebin}, only four out of the ten scanners were in our set of correct scanners, namely \texttt{Avira}, \texttt{ESET-NOD32}, \texttt{McAfee}, and \texttt{Sophos}. 
Apart from referring to the ten scanners they chose as \emph{common}, Arp et al.\ did not mention why they chose those ten scanners. 
We assume that common means popular and trustworthy. 
The results we obtained from our measurement do not undermine this assumption because these results are based on the versions of the \emph{Drebin} scanners used by \texttt{VirusTotal}. 
The example of \texttt{BitDefender} we gave earlier shows that such versions do not always reflect the performance of a scanner in reality. 
So, the results we present in this section (i.e., the list of correct \texttt{VirusTotal} scanners), are confined to \texttt{VirusTotal} and the versions it uses, which does not hinder the objective of this paper, viz.\ analyzing \texttt{VirusTotal} to build accurate \gls{ml}-based labeling strategies. 

%\subsection{Correctness and Consistency on Other Datasets}
%\label{subsec:correctness_other}
We found that a set of \CorrectScannersCount{} \texttt{VirusTotal} scanners had average correctness rates of at least 90\% between \earliestDate{} and \latestDate{}. 
Our concern in this section is whether the same set of \texttt{VirusTotal} scanners persists on other datasets. 
So, we retrieved the set of scanners that maintained correctness rates of 90\% or higher over a period of time for the \emph{AMD+GPlay}, \emph{GPlay}, \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets. 
Since we downloaded the apps in the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets after downloading apps in the \emph{AMD+GPlay} dataset, we started re-scanning and downloading their latest \texttt{VirusTotal} scan reports at later points in time, viz.\ starting from \interDate{} instead of \earliestDate{}. 
So, to perform an objective measurement, we retrieved the list of correct \texttt{VirusTotal} scanners for the \emph{AMD+GPlay}, \emph{Hand-Labeled}, \emph{Hand-Labeled 2019} datasets within the same time period, namely between \interDate{} and \latestDate{}. 

As seen in \autoref{tab:correct_scanners_otherdatasets}, the set of \texttt{VirusTotal} scanners that have correctness rates of at least 90\% differ from one dataset to another, despite being based on scan reports downloaded within the same period. 
Only a set of five scanners continued to be the most correct in labeling apps in all datasets, viz.\ \texttt{ESET-NOD32}, \texttt{Fortinet}, \texttt{Ikarus}, \texttt{McAfee}, and \texttt{SymantecMobileInsight}. 
As for the \emph{GPlay} dataset, a total of 58 correct scanners were found to be correct, which we could not fit in the table. 

%\bgroup
%\def\arraystretch{1.5}
\begin{table*}[]
%\begin{sidewaystable}
\centering
\caption{The set of \texttt{VirusTotal} scanners that had correctness rates of at least 90\% between \interDate{} and \latestDate{}. Emboldened scanners depict the intersection of the sets of correct scanners of the four datasets.}
\label{tab:correct_scanners_otherdatasets}
%\small
\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}|ccc|@{}}
\toprule
Dataset & Scanner(s) & Total \\ \hline
\emph{AMD} & \begin{tabular}[c]{@{}c@{}}\texttt{Avira}, \texttt{CAT-QuickHeal}, \texttt{DrWeb}, \textbf{\texttt{ESET-NOD32}}, \texttt{F-Secure}, \\ \textbf{\texttt{Fortinet}}, \textbf{\texttt{Ikarus}}, \texttt{MAX}, \textbf{\texttt{McAfee}}, \texttt{NANO-Antivirus}, \\ \texttt{Sophos}, \textbf{\texttt{SymantecMobileInsight}} \end{tabular} & 12 \\ \hline

\emph{AMD+GPlay} & \begin{tabular}[c]{@{}c@{}}\texttt{AhnLab-V3}, \texttt{Avira}, \texttt{CAT-QuickHeal}, \texttt{Comodo}, \texttt{Cyren}, \\ \texttt{DrWeb}, \textbf{\texttt{ESET-NOD32}}, \texttt{F-Secure}, \textbf{\texttt{Fortinet}}, \\ \textbf{\texttt{Ikarus}}, \texttt{K7GW}, \texttt{MAX}, \textbf{\texttt{McAfee}},  \texttt{NANO-Antivirus}, \\ \texttt{Sophos}, \textbf{\texttt{SymantecMobileInsight}}, \texttt{TheHacker}, \texttt{Trustlook}\end{tabular} & 18 \\ \hline

\emph{Hand-Labeled} & \begin{tabular}[c]{@{}c@{}}\texttt{AhnLab-V3}, \texttt{CAT-QuickHeal}, \texttt{Cyren}, \textbf{\texttt{ESET-NOD32}}, \textbf{\texttt{Fortinet}}, \textbf{\texttt{Ikarus}}, \\ \texttt{K7GW}, \textbf{\texttt{McAfee}}, \texttt{Sophos}, \textbf{\texttt{SymantecMobileInsight}}, \texttt{Trustlook}\end{tabular} & 11 \\ \hline

\emph{Hand-Labeled 2019} & \begin{tabular}[c]{@{}c@{}}\texttt{Ad-Aware}, \texttt{AegisLab}, \texttt{AhnLab-V3}, \texttt{Alibaba}, \texttt{Arcabit}, \\ \texttt{Avast-Mobile}, \texttt{BitDefender}, \texttt{ClamAV}, \texttt{Cyren}, \texttt{DrWeb}, \\ \textbf{\texttt{ESET-NOD32}}, \texttt{Emsisoft}, \texttt{F-Secure}, \texttt{FireEye}, \textbf{\texttt{Fortinet}}, \\ \texttt{GData}, \textbf{\texttt{Ikarus}}, \texttt{Jiangmin}, \texttt{K7AntiVirus}, \texttt{K7GW}, \\ \texttt{Kaspersky}, \texttt{Kingsoft}, \texttt{MAX}, \texttt{MalwareBytes}, \textbf{\texttt{McAfee}}, \\ \texttt{McAfee-GW-Edition}, \texttt{MicroWorld-eScan}, \texttt{Microsoft}, \texttt{NANO-Antivirus}, \texttt{Qihoo-360}, \\ \texttt{SUPERAntiSpyware}, \textbf{\texttt{SymantecMobileInsight}}, \texttt{Trustlook}, \texttt{ViRobot}, \texttt{Yandex}, \\ \texttt{ZoneAlarm}, \texttt{Zoner}\end{tabular} & 37 \\ \bottomrule
\end{tabular}}
\end{table*}
%\end{sidewaystable}
%\egroup

We made the following observations based on the results in the table. 
Firstly, the set of \texttt{VirusTotal} scanners that were found to be the most correct in labeling apps in the \emph{AMD} dataset between \earliestDate{} and \latestDate{} changed, both, in terms of number (i.e., \CorrectScannersCount{} versus 12), and scanners. 
Secondly, we noticed that adding more benign apps to a dataset increases the number of scanners found to be correct. 
In other words, the more malicious apps in a dataset, the lower the number of correct scanners. 
For example, adding the scan reports of apps in the \emph{GPlay} dataset to their \emph{AMD} counterparts increases the number of scanners found to be correct between \interDate{} and \latestDate{} from 12 scanners to 18 scanners. 
On a smaller scale, one can notice the same pattern in the \emph{Hand-Labeled} and \emph{Hand-Labeled 2019} datasets. 
Since the former dataset has less benign apps and more malicious ones (i.e., 76 benign versus 24 malicious), the number of scanners found to be correct is less than that for the latter dataset that has 90 benign apps and only 10 malicious ones. 

What we learned from this measurement is that the set of \texttt{VirusTotal} scanners that are correct over time is not universal and changes depending on (a) the dataset itself and its composition in terms of benign and malicious apps, and (b) the time period within which the \texttt{VirusTotal} scan reports were gathered. 
One of the reasons behind this change is the fact that \texttt{VirusTotal} may suddenly change the versions of scanners it uses in its scan reports, as seen with the cases of \texttt{BitDefender} and \texttt{Panda}.
However, according to our measurements, a small set of \texttt{VirusTotal} scanners appear to be consistently correct across different datasets, time periods, and malware types. 
In this case, this set comprised a mere of five scanners out of the 60 used by \texttt{VirusTotal}. 

==> backup/time.tex <==
\section{Stability of \texttt{VirusTotal} Scanners}
\label{sec:time}
Researchers have found that--courtesy of the changing performance of scanners--\texttt{VirusTotal}'s scan reports are dynamic and change over time ~\cite{lalande2018challenges,hurier2017euphony,kantchelian2015better,mohaisen2014av}, which we demonstrated in \autoref{subsec:preliminaries_motivation} and in the previous section. 
This dynamic nature of scan reports is expected to alter the labels given to apps, which might result in unreliable detection results. 
Consequently, the research community has attempted to estimate whether \texttt{VirusTotal} scan reports eventually stabilize and the period it takes them to stabilize ~\cite{pendlebury2019,miller2016reviewer,kantchelian2015better}. 
That is, we attempt to answer the research question: 

\begin{tcolorbox}[colback=white]%[title=\textbf{RQ3},colback=white]
	\footnotesize
	\textbf{RQ2} \RQtwo
\end{tcolorbox}

Within the context of Windows-based malware, Miller et al.\ suggested that it takes approximately \emph{one year} for \texttt{VirusTotal} scan reports to stabilize \cite{miller2016reviewer}, whereas Kantchelian et al.\ argued in \cite{kantchelian2015better} that this period can be as brief as \emph{four weeks} \cite{kantchelian2015better}. 
Unfortunately, both research efforts did not provide a definition of \emph{stability} or how it can be measured. 
The most intuitive definition of stability is in terms of the number \texttt{VirusTotal} scanners deeming an app as malicious (i.e., \emph{positives}): if this number did not change after reanalysis, then the app's scan report can be assumed to have stabilized, even if the scanners that deem the app malicious have changed. 
This difference in \emph{positives} is captured by another attribute in a \texttt{VirusTotal} scan report, viz.\ \emph{positives\_delta}. 
So, the period it takes for a scan report to stabilize can be measured as the difference between the date on which \emph{positives\_delta} converged to zero and the date on which the app was first seen on \texttt{Virustotal}. 
For each app, we can iterate over its \texttt{VirusTotal} scan reports that depict re-analyses at different points in time and check the value of the  \emph{positives\_delta} field. 
Once the value reaches zero, we can assume that the scan report has stabilized and calculate the time between the first time the app has been seen on \texttt{VirusTotal} and the date of the scan report in which \emph{positives\_delta} is equal to zero (i.e., the difference between the \emph{scan\_date} and \emph{first\_seen} attributes in the scan report.

With that in mind, consider the data in \autoref{tab:example_hesitant}, which belongs to an app of type \texttt{Ransom} that was first seen on \texttt{VirusTotal} on  May 11$^{th}$, 2015.
According to the \emph{positives\_delta==0} criterion, the app appeared to have stabilized on January 8$^{th}$, 2019 (i.e., four years after being first seen on \texttt{VirusTotal}). 
However, reanalyzing the app after three months (i.e., on April 12$^{th}$) indicates that eight scanners seized to deem the app as malicious, rendering the value of \emph{positives\_delta} to -8. 
The number of \texttt{VirusTotal} scanners deeming the app as malicious (\emph{positives}) and the total number of scanners that scanned the app (\emph{total}) continue to fluctuate across different re-analysis points that are merely two weeks apart. 
This example suggests that a definition of stability according to the criterion \emph{positives\_delta==0} is inadequate, given the dynamicity of \texttt{VirusTotal}.  
In general, the alternative definition of stability should refrain from defining stability in terms of a specific value or attribute (e.g., \emph{positives\_delta==0} or \emph{total==61}). 

\bgroup
\def\arraystretch{1.0}
\begin{table}[]
\centering
\caption[The evolution of \texttt{5cfda85debe5e9a7341b4eeed01d92807ed29552}'s scan reports]{The evolution of the \texttt{VirusTotal} scan reports for \texttt{5cfda85debe5e9a7341b4eeed01d92807ed29552} between December 3$^{rd}$, 2018 and \latestDate{}. The grayed column depicts the date on which the app's scan report appeared to have stabilized with \emph{positives\_delta} converging to zero.}
\label{tab:example_hesitant}
%\small
\tiny
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccccccccccccccc|}%c|}
\cline{2-16}
 & \rotatebox[origin=c]{90}{2018-12-03 } & \cellcolor{gray!25}\rotatebox[origin=c]{90}{2019-01-08} & \rotatebox[origin=c]{90}{2019-04-12} & \rotatebox[origin=c]{90}{2019-04-25} & \rotatebox[origin=c]{90}{2019-05-09} & \rotatebox[origin=c]{90}{2019-05-23} & \rotatebox[origin=c]{90}{2019-06-07} & \cellcolor{gray!25}\rotatebox[origin=c]{90}{2019-06-21} & \rotatebox[origin=c]{90}{2019-07-05} & \rotatebox[origin=c]{90}{2019-07-19} & \rotatebox[origin=c]{90}{2019-08-02} & \rotatebox[origin=c]{90}{2019-08-16} & \rotatebox[origin=c]{90}{2019-08-30} & \rotatebox[origin=c]{90}{2019-09-13} & \cellcolor{gray!25}\rotatebox[origin=c]{90}{2019-09-27} \\ \toprule %& \rotatebox[origin=c]{90}{2019-10-11} \\ \toprule
\multicolumn{1}{|c|}{\emph{positives}} & 39 & \cellcolor{gray!25}39 & 31 & 33 & 34 & 30 & 32 & \cellcolor{gray!25}32 & 31 & 32 & 33 & 25 & 30 & 29 & \cellcolor{gray!25}29 \\ \hline %& \xmark \\ \hline
\multicolumn{1}{|c|}{\emph{total}} & 60 & \cellcolor{gray!25}58 & 57 & 61 & 61 & 60 & 61 & \cellcolor{gray!25}62 & 60 & 60 & 61 & 56 & 60 & 59 & \cellcolor{gray!25}59 \\ \hline %& \xmark \\ \hline
\multicolumn{1}{|c|}{\emph{positives}:\emph{total}} & 0.65 & \cellcolor{gray!25}0.67 & 0.54 & 0.54 & 0.55 & 0.5 & 0.52 & \cellcolor{gray!25}0.51 & 0.51 & 0.53 & 0.54 & 0.44 & 0.50 & 0.49 & \cellcolor{gray!25}0.49 \\ \hline %& \xmark \\ \hline
\multicolumn{1}{|c|}{\emph{positives\_delta}} & 2 & \cellcolor{gray!25}0 & -8 & 2 & 1 & -3 & 2 & \cellcolor{gray!25}0 & -1 & 1 & 1 & -7 & 5 & -1 & \cellcolor{gray!25}0 \\ \bottomrule %& \xmark \\ \bottomrule
\end{tabular}}
\end{table}
\egroup

Through the measurements we performed in \autoref{sec:correctness}, we found that a subset of \texttt{VirusTotal} scanners are correct in labeling apps in the \emph{AMD} dataset more often than others over a period of time between \earliestDate{} and \latestDate{}. 
The continuity of correctly labeling apps, we argue, implies the stability of labels.
So, we suggest defining scan reports' stability in terms of the verdicts given by the most correct \texttt{VirusTotal} scanners. 
If we can show that a \texttt{VirusTotal} scanner maintains the first label it assigns to an app over an extended period of time, then we can bypass time-based definitions of stability altogether, and rely on the verdict given by such a scanner.

We focused on the verdicts given by the \CorrectScannersCount{} scanners that we deemed as correct on the \emph{AMD} apps between \earliestDate{} and \latestDate{}.
To check whether those scanners are also stable, we should compare the labels given by the scanners to apps in the \emph{AMD} dataset ever since they were first seen on \texttt{VirusTotal}, which is infeasible given that we do not possess scan reports older than \earliestDate{}. 
With the help of members of the research community, we acquired scan reports for 13,149 (53\%) of apps in the \emph{AMD} dataset whose scan dates predate \earliestDate{}. 
To test Miller et al.'s one-year hypothesis, we further filtered those apps to focus on those for which the difference between their \emph{scan\_date}s and the time they were \emph{first\_seen} on \texttt{VirusTotal} is at most 12 months, which brought the number of apps to 8,864. 
Using those apps, we calculated the number of times each scanner maintained the same verdict it \emph{initially} assigned to the apps. 
For example, if in the oldest scan report we possess for an app ($\alpha$), the scanner \texttt{ESET-NOD32} labeled ($\alpha$) as malicious, we calculate the percentage of times \texttt{ESET-NOD32} labeled ($\alpha$) as such in more recent scan reports. 
We refer to this value as \emph{certainty} and define it as the variance of the labels given to apps by \texttt{VirusTotal} scanners approaching zero over a period of time. 
Following the example above, say \texttt{ESET-NOD32} had the labels $\lbrace \textcolor{ACMRed}{\texttt{malicious}}, \textcolor{ACMGreen}{\texttt{benign}}, \textcolor{ACMRed}{\texttt{malicious}}, \textcolor{ACMRed}{\texttt{malicious}}\rbrace$ for ($\alpha$), the certainty percentage will be three (i.e., counts of malicious), divided by a total of four labels yielding a percentage of 75\%. 

We found that the \CorrectScannersCount{} scanners we use maintained the same initial label until \latestDate{} 98.86$\pm$1.16\% of the time on average. 
We repeated the same measurement, decreasing the allowed difference between the \emph{scan\_date} and \emph{first\_seen} to six months, three months, one month \cite{kantchelian2015better}, and one week. 
While the number of apps that meet the criterion was reduced to 7,514, 6,910, 6,413, and 5,981, respectively, the persistence and certainty of the \CorrectScannersCount{} remained almost the same. 
For example, the average certainty scores of these scanners in a difference of one month and one week were 98.82$\pm$1.25\% and 98.83$\pm$1.26\%, respectively.

It is important to make the distinction between an app being analyzed by an antiviral scanner and being \emph{first\_seen} or uploaded to \texttt{VirusTotal}. 
The \emph{first\_seen} depicts the date on which the app was uploaded to \texttt{VirusTotal} for analysis. 
However, an app can be developed and analyzed by commercial versions of \texttt{VirusTotal} scanners years before it is to be seen on the platform (e.g., once an independent researcher uploads the app for analysis). 
We found that the malicious apps in the \emph{AMD} dataset have a mean, median, and standard deviation difference between the \emph{first\_seen} dates and the dates on which their APK archives were last modified (i.e., \emph{dex\_date}), of 153.6 days, 21 days, and 685.6 days. 
This means that a newly-developed Android malicious app can exist in the wild for two years before it is \emph{uploaded} to \texttt{VirusTotal} for analysis. 
However, this does not imply that scanners take two years to discover, analyze, and label Android apps. 
Some researchers, such as Zetter \cite{zetter2014countdown}, found that antiviral scanners aspire to shorten the time between discovering a new app in the wild and labeling it to periods as short as one day. 
So, we extended the previous measurements to measure the time it takes \texttt{VirusTotal} scanners to devise persistent and certain labels for Android apps based on the \texttt{dex\_date}. 
We focus on \emph{AMD} apps in which the difference between the \emph{scan\_date} and \emph{dex\_date} is less than or equal a year, six months, three months, one month, and one week. 
With a difference of one year, the certainty score of the scanners was 98.78$\pm$1.29\% against the 6,566 apps that fit this new criterion. 
The score for a difference of one week was very similar for 1,367 apps, namely 98.51$\pm$1.59\%.

What we have shown so far is that \texttt{VirusTotal} scanners that prove to be correct over periods of time can be trusted \emph{not} to change the verdicts they initially give to apps even within one week of the apps' release. 
This may relieve the community from the burden of having to devise a metric or a time period within which the \texttt{VirusTotal} scan reports stabilize. 
That is, instead of relying on attributes, such as \emph{positives} or \emph{total}, to infer the stability of scan reports, researchers can adopt the verdicts given by a subset of \texttt{VirusTotal} scanners because they are unlikely to change in the future. 
However, it is worth mentioning that any definition of stability, including this one, suffers from two limitations. 
Firstly, there is no absolute guarantee that the performance of a \texttt{VirusTotal} scanner will continue to be the same, either because of technical difficulties suffered by an antiviral software company or because of \texttt{VirusTotal}'s utilization of different versions of a scanner, as seen in the case of \texttt{BitDefender}.
Secondly, any definition of stability does not guarantee correctness. 
Over the past three years, we tracked the verdicts given by \texttt{VirusTotal} scanners to a repackaged, malicious version\footnote{aa0d0f82c0a84b8dfc4ecda89a83f171cf675a9a} of the \texttt{K9 Mail} open source app \cite{k9mail2019} that has been developed by one of our students during a practical course. 
Despite being a malicious app of type \texttt{Ransom}, the scanners continued to unanimously deem the app as benign since February 8$^{th}$, 2017, even after analyzing and re-scanning the app. 
